Using Depth for Pixel-Wise Detection of Adversarial Attacks in Crowd Counting

State-of-the-art methods for counting people in crowded scenes rely on deep networks to estimate crowd density. While effective, deep learning approaches are vulnerable to adversarial attacks, which, in a crowd-counting context, can lead to serious security issues. However, attack and defense mechanisms have been virtually unexplored in regression tasks, let alone for crowd density estimation. In this paper, we investigate the effectiveness of existing attack strategies on crowd-counting networks, and introduce a simple yet effective pixel-wise detection mechanism. It builds on the intuition that, when attacking a multitask network, in our case estimating crowd density and scene depth, both outputs will be perturbed, and thus the second one can be used for detection purposes. We will demonstrate that this significantly outperforms heuristic and uncertainty-based strategies.

==> fig/depth_detection.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure}[htbp]
\centering
 \includegraphics[width=0.5\linewidth]{images/depth_detection.pdf}
\vspace{-3mm}
  \caption{ {\bf Detection accuracy on MICC.} We report the detection accuracy for depth values tampered with different strengths.
}
  \label{fig:depth_detection}
  \end{figure}


==> fig/venice.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure}[t]
\centering
 \includegraphics[width=0.5\linewidth]{images/venice.jpg}
\vspace{-3mm}
  \caption{ {\bf Example image from {\bf Venice}.} In the {\bf Venice} dataset, each image is provided with a perspective map, which is computed from the grid-like ground pattern.
}
  \label{fig:venice}
  \end{figure}


==> table/whitebox.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{table}
  \centering
  \scalebox{0.8}{
\begin{tabular}{ |p{1cm}|c|c|c|c|}

  \hline
  $\lambda$  & \FGSMUE{1}& \FGSMTE{1} & \FGSMUE{19}& \FGSMTE{19}  \\
  \hline
  0.01 & {\bf 0.52} & {\bf 0.51} & {\bf 0.45} & {\bf 0.47}  \\
  \hline
  1.0  & 0.41 & 0.38& 0.36& 0.36 \\
  \hline
  100.0 &0.36 & 0.33& 0.30& 0.31\\
  \hline
  \end{tabular}
  }
  \caption{{\bf Detection accuracy for different $\lambda$ values in white-box attacks on ShanghaiTechRGBD}}
  \label{tab:whitebox}
\end{table}
